Defending against Reconstruction Attack in Vertical Federated Learning

Recently researchers have studied input leakage problems in Federated Learning (FL) where a malicious party can reconstruct sensitive training inputs provided by users from shared gradient. It raises concerns about FL since input leakage contradicts the privacy-preserving intention of using FL. Despite a relatively rich literature on attacks and defenses of input reconstruction in Horizontal FL, input leakage and protection in vertical FL starts to draw researcher's attention recently. In this paper, we study how to defend against input leakage attacks in Vertical FL. We design an adversarial training-based framework that contains three modules: adversarial reconstruction, noise regularization, and distance correlation minimization. Those modules can not only be employed individually but also applied together since they are independent to each other. Through extensive experiments on a large-scale industrial online advertising dataset, we show our framework is effective in protecting input privacy while retaining the model utility.

==> tex/back.tex <==
\section{Background: Vertical Federated Learning (should be deleted)}
\kevin{Maybe we can remove or shorten this section. It's FL workshop, everyone should know vFL?}

For simplicity, we consider two parties split learning a model for a binary classification problem over the domain $\calX \times \cbrck{0, 1}$ as an example. Here the passive and active parties want to learn a composition model $h \circ f$ jointly, where the raw features $X$ and $f: \calX \to \Real^d$ are stored the passive party side while the labels $y$ and $h: \Real^d \to \Real$ is on the active party side. Let $\ell = h(f(X))$ be the logit of the positive class where the positive class's predicted probability is given by the sigmoid function as follows: $\widetilde{p}_1 = 1/(1 + \exp(-\ell))$. The loss of the model is given by the cross entropy $L = \log(1 + \exp(-\ell)) + (1 - y)\ell$. During the model inference, the passive party computes $f(X)$ and sends it to the active party who will then compute the rest of computation (Forward in Table \ref{tab:model_training}). \footnote{For the simplifying of the notation and derivation, we add no additional features in the active party to compute the logit.} 

To train the model using gradient descent, the active party starts the gradient computation process by first computing the gradient of the loss with respect to the logit $\frac{dL}{d\ell} = (\widetilde{p}_1 - y)$. Using chain rule, the active party can then compute the gradient of $L$ with respect to $h$'s parameters through $\ell$. In order to also allow the passive party to learn $f$, the active party also computes the gradient of $L$ with respect to the input of the function $h$. We denote this gradient by \linelabel{eq:g} $g \coloneqq \nabla_{f(X)} L = (\widetilde{p}_1 - y) \nabla_a h(a) \vert_{a = f(X)} \in \Real^d$  (last equality by chain rule). After receiving $g$ sent from the active party, the passive party can compute the gradient of $L$ with respect to $f$'s parameters (Backward in Table \ref{tab:model_training}). 

% \newcommand{\pp}{c}
  \begin{table*}[h!!]
  \centering
%   \begin{center}
    \scriptsize
    \begin{tabular}{ \pp \pp \pp \pp \pp \pp \pp \pp \pp \pp }
      { Forward:} & $X$ & $\xrightarrow{\bm{f}}$ & $\bm{f}(X)$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longrightarrow}$ & $\bm{f}(X)$ & $\xrightarrow{\bm{h}}$ &$\ell$ & $\rightarrow$ & $\stackrel{\stackrel{\mbox{$y$}}{\downarrow}}{L}$ \\
      { Backward:} & & & $g$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longleftarrow}$ & $g $ & $\leftarrow$ & $\frac{dL}{dl} = (\tilde{p_1} - y)$ & $\leftarrow$ & $1$ \\
      & & & $\downarrow$ & & & & $\downarrow$ & & \\
      & & & $f$'s param & & & & $h$'s param & & 
    \end{tabular}
%   \end{center}
    \caption{Computation and communication diagram of model training ($\leftarrow$ and $\downarrow$ represent gradient computation using chain rule)}
    \label{tab:model_training}
  \end{table*}

When $B$ examples are forwarded as a batch, the communicated features $f(X)$ and gradients $g$ will both be matrices of shape $\Real^{B \times d}$ with each row belonging to a specific example in the batch. It is important to note that here the gradients as rows of the matrix are gradients of the loss with respect to different examples' intermediate computation results but not the model parameters; therefore, no averaging over or shuffling of the rows of the matrix can be done prior to communication for the sake of correct gradient computation of $f$'s parameters on the passive party side.

Previous work ~\cite{understandingDeepImage2015, LiDeepObfuscator, zhu2019dlg} have shown that $f(X)$ still contain rich information which can breach users’ privacy. Adversary attackers can leverage $f(X)$ to recover the raw features and infer private attributes, such as gender and age.

